Your Co-Workers Matter: Evaluating Collaborative Capabilities of Language Models in Blocks World

Language agents that interact with the world on their own have great potential for automating digital tasks. While large language model (LLM) agents have made progress in understanding and executing tasks such as textual games and webpage control, many real-world tasks also require collaboration with humans or other LLMs in equal roles, which involves intent understanding, task coordination, and communication. To test LLM's ability to collaborate, we design a blocks-world environment, where two agents, each having unique goals and skills, build a target structure together. To complete the goals, they can act in the world and communicate in natural language. Under this environment, we design increasingly challenging settings to evaluate different collaboration perspectives, from independent to more complex, dependent tasks. We further adopt chain-of-thought prompts that include intermediate reasoning steps to model the partner's state and identify and correct execution errors. Both human-machine and machine-machine experiments show that LLM agents have strong grounding capacities, and our approach significantly improves the evaluation metric.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/task.tex <==
%Typically, these LLMs are trained to assist without stipulating specific requirements~\cite{DBLP:conf/chi/WangSGJ021}. 
%Hence, the capability of agents to adeptly persuade and negotiate with humans in pursuit of their objectives remains a challenge.

% While LLMs have achieved remarkable success in executing tasks within single-agent frameworks~\cite{DBLP:journals/corr/abs-2305-14628}. Within such controlled and unambiguous environments, LLMs excel, allowing for the precise delineation and pursuit of objectives.
% However, the transition from single-agent to multi-agent settings introduces a series of intricate challenges and complexities, predominantly due to the inherently heterogeneous nature of the agents involved~\cite{DBLP:journals/ai/SlaneyT01}. Each agent, equipped with divergent goals, capabilities, and decision-making strategies, necessitates the orchestration of advanced collaboration and communication mechanisms to harmonize diverse and potentially conflicting intentions and actions.
% The multifaceted nature of multi-agent environments necessitates the alignment of varied agent goals and optimization of communication and actions for collaboration. Given these challenges, a dedicated evaluative platform is crucial to investigate Large Language Models' (LLMs) collaborative capabilities in such intricate settings, thus offering insights into their adaptability and performance in environments with divergent agent goals and actions.


%\chen{Moved from section 2.2}
% Communication holds paramount importance in multi-agent collaborations. To thoroughly investigate the dynamics of communication within such settings, an environment with rich information exchange mechanisms is indispensable. 

% In multi-agent collaboration, agents often encounter intricate challenges that are rarely observed in single-agent paradigms. These challenges primarily arise due to the heterogeneous nature of agents involved, each possessing unique goals, capabilities, and decision-making strategies~\cite{DBLP:journals/ai/SlaneyT01}. The presence of multiple agents mandates the development of sophisticated collaboration and communication mechanisms to harmonize divergent agent intentions and actions. Multi-agent collaboration introduces complexities related to consensus achievement and conflict resolution, both critical to maintaining synchrony and preventing counterproductive actions~\cite{Horling2004}. This requires agents to negotiate, share strategic information adaptively, and synchronize actions to uphold system coherence and facilitate the attainment of shared objectives.

% LLMs have been proven to be effective in the single-agent tasks~\cite{DBLP:journals/corr/abs-2305-14628}. However, LLMs' capabilities in the multi-agent collaboration has not been extensively studies. 




==> tables/human-model.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!h]
\begin{center}
    
\begin{tabular}{lllrrr}
\hline
\multicolumn{1}{|l|}{Model}                    & \multicolumn{1}{l|}{Method}                    & \multicolumn{1}{l|}{Task Type} & \multicolumn{1}{l|}{Success Rate} & \multicolumn{1}{l|}{Task Workload Balance} & \multicolumn{1}{l|}{Time} \\ \hline
\multicolumn{1}{|l|}{\multirow{6}{*}{GPT-4}}   & \multicolumn{1}{l|}{\multirow{3}{*}{Baseline}} & \multicolumn{1}{l|}{Unrelated} & \multicolumn{1}{r|}{91.67\%}      & \multicolumn{1}{r|}{0.41}                  & \multicolumn{1}{r|}{10.7} \\ \cline{3-6} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{Related}   & \multicolumn{1}{r|}{66.67\%}      & \multicolumn{1}{r|}{0.38}                  & \multicolumn{1}{r|}{9.4}  \\ \cline{3-6} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{Dependent} & \multicolumn{1}{r|}{62.50\%}      & \multicolumn{1}{r|}{0.33}                  & \multicolumn{1}{r|}{9.1}  \\ \cline{2-6} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{l|}{\multirow{3}{*}{Ours}}     & \multicolumn{1}{l|}{Unrelated} & \multicolumn{1}{r|}{91.67\%}      & \multicolumn{1}{r|}{0.43}                  & \multicolumn{1}{r|}{9.5}  \\ \cline{3-6} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{Related}   & \multicolumn{1}{r|}{87.50\%}      & \multicolumn{1}{r|}{0.41}                  & \multicolumn{1}{r|}{8.7}  \\ \cline{3-6} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{Dependent} & \multicolumn{1}{r|}{79.17\%}      & \multicolumn{1}{r|}{0.4}                   & \multicolumn{1}{r|}{8.8}  \\ \hline
\multicolumn{1}{|l|}{\multirow{6}{*}{GPT-3.5}} & \multicolumn{1}{l|}{\multirow{3}{*}{Baseline}} & \multicolumn{1}{l|}{Unrelated} & \multicolumn{1}{r|}{70.83\%}      & \multicolumn{1}{r|}{0.43}                  & \multicolumn{1}{r|}{12.1} \\ \cline{3-6} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{Related}   & \multicolumn{1}{r|}{41.67\%}      & \multicolumn{1}{r|}{0.39}                  & \multicolumn{1}{r|}{10.7} \\ \cline{3-6} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{Dependent} & \multicolumn{1}{r|}{37.50\%}      & \multicolumn{1}{r|}{0.38}                  & \multicolumn{1}{r|}{10.6} \\ \cline{2-6} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{l|}{\multirow{3}{*}{Ours}}     & \multicolumn{1}{l|}{Unrelated} & \multicolumn{1}{r|}{79.17\%}      & \multicolumn{1}{r|}{0.42}                  & \multicolumn{1}{r|}{11.9} \\ \cline{3-6} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{Related}   & \multicolumn{1}{r|}{54.17\%}      & \multicolumn{1}{r|}{0.41}                  & \multicolumn{1}{r|}{9.6}  \\ \cline{3-6} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{Dependent} & \multicolumn{1}{r|}{58.33\%}      & \multicolumn{1}{r|}{0.41}                  & \multicolumn{1}{r|}{9.8}  \\ \hline
                                               &                                                &                                & \multicolumn{1}{l}{}              & \multicolumn{1}{l}{}                       & \multicolumn{1}{l}{}     
\end{tabular}

\caption{Experiment results on human-model settings}
\label{tab:human-model}
\end{center}

\end{table*}



==> tables/model-only.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\begin{center}

\begin{tabular}{|l|l|l|r|r|r|}
\hline
Model                    & Method                               & Task Type & \multicolumn{1}{l|}{Success Rate} & \multicolumn{1}{l|}{W.B.} & \multicolumn{1}{l|}{Time} \\ \hline
\multirow{9}{*}{GPT-4}   & \multirow{3}{*}{Baseline}            & Unrelated & 87.50\%                           & 0.4                       & 9.5                       \\ \cline{3-6} 
                         &                                      & Related   & 62.50\%                           & 0.38                      & 10.9                      \\ \cline{3-6} 
                         &                                      & Dependent & 50.00\%                           & 0.33                      & 10.4                      \\ \cline{2-6} 
                         & \multirow{3}{*}{Ours w/o Reflection} & Unrelated & 91.67\%                           & 0.41                      & 9.3                       \\ \cline{3-6} 
                         &                                      & Related   & 79.17\%                           & 0.4                       & 9.1                       \\ \cline{3-6} 
                         &                                      & Dependent & 70.83\%                           & 0.39                      & 9.3                       \\ \cline{2-6} 
                         & \multirow{3}{*}{Ours}                & Unrelated & 87.50\%                           & 0.41                      & 9.4                       \\ \cline{3-6} 
                         &                                      & Related   & 87.50\%                           & 0.42                      & 8.7                       \\ \cline{3-6} 
                         &                                      & Dependent & 79.17\%                           & 0.4                       & 8.3                       \\ \hline
\multirow{9}{*}{GPT-3.5} & \multirow{3}{*}{Baseline}            & Unrelated & 70.83\%                           & 0.39                      & 11.3                      \\ \cline{3-6} 
                         &                                      & Related   & 33.33\%                           & 0.35                      & 12.1                      \\ \cline{3-6} 
                         &                                      & Dependent & 25.00\%                           & 0.34                      & 12.4                      \\ \cline{2-6} 
                         & \multirow{3}{*}{Ours w/o Reflection} & Unrelated & 75.00\%                           & 0.39                      & 11.2                      \\ \cline{3-6} 
                         &                                      & Related   & 50.00\%                           & 0.37                      & 10.9                      \\ \cline{3-6} 
                         &                                      & Dependent & 45.83\%                           & 0.38                      & 10.7                      \\ \cline{2-6} 
                         & \multirow{3}{*}{Ours}                & Unrelated & 75.00\%                           & 0.4                       & 11/2                      \\ \cline{3-6} 
                         &                                      & Related   & 45.83\%                           & 0.39                      & 10.3                      \\ \cline{3-6} 
                         &                                      & Dependent & 54.17\%                           & 0.41                      & 9.8                       \\ \hline
\end{tabular}

\caption{Experiment results on model-only settings}
\label{tab:model-only}
\end{center}
\end{table*}

==> tables/preliminary.tex <==
\begin{table}[]
    \begin{center}
    \begin{tabular}{|l|r|r|r|}
    \hline
    Model   & \multicolumn{1}{l|}{Part I } & \multicolumn{1}{l|}{Part II } & \multicolumn{1}{l|}{Part III} \\ \hline
    GPT-3.5 & 80.0\%                                          & 73.3\%                                     & 66.7\%                                     \\ \hline
    GPT-4   & 86.7\%                                          & 93.3\%                                     & 86.7\%                                     \\ \hline
    \end{tabular}
    \caption{Experiment results on the grounding tasks. The all result values are the success rates of the tasks.\chen{Make it a figure.}}
\label{tab:grounding}
\end{center}
    \end{table}
